DistDF: Time-Series Forecasting Needs Joint-Distribution Wasserstein Alignment

Training time-series forecasting models requires aligning the conditional distribution of model forecasts with that of the label sequence. The standard direct forecast (DF) approach resorts to minimizing the conditional negative log-likelihood, typically estimated by the mean squared error. However, this estimation proves biased when the label sequence exhibits autocorrelation. In this paper, we propose DistDF, which achieves alignment by minimizing a distributional discrepancy between the conditional distributions of forecast and label sequences. Since such conditional discrepancies are difficult to estimate from finite time-series observations, we introduce a joint-distribution Wasserstein discrepancy for time-series forecasting, which provably upper bounds the conditional discrepancy of interest. The proposed discrepancy is tractable, differentiable, and readily compatible with gradient-based optimization. Extensive experiments show that DistDF improves diverse forecasting models and achieves leading performance. Code is available at https://anonymous.4open.science/r/DistDF-F66B.

==> table_hparam2.tex <==



\begin{table}[t]
\begin{minipage}[t]{0.495\textwidth}
\makeatletter\def\@captype{table}
\renewcommand{\arraystretch}{1} \setlength{\tabcolsep}{4.7pt} \scriptsize
\centering
\renewcommand{\multirowsetup}{\centering}
\begin{threeparttable}
\caption{Varying $\gamma$ results of TimeBridge}\label{tab:sensi-alpha}
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{$\gamma$} & \multicolumn{2}{c}{ETTh2} & \multicolumn{2}{c}{ECL} & \multicolumn{2}{c}{Weather} \\
    \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
    & MSE & MAE & MSE & MAE & MSE & MAE \\
    \midrule
    0 & 0.377 & 0.403 & 0.176 & 0.271 & 0.252 & 0.277  \\
    0.001 & 0.378 & 0.402 & 0.172 & 0.267 & 0.250 & \subbst{0.276}  \\
    0.002 & 0.377 & 0.402 & 0.173 & 0.267 & 0.250 & 0.276  \\
    0.005 & 0.376 & 0.401 & \bst{0.172} & \bst{0.267} & 0.250 & \bst{0.276}  \\
    0.01 & 0.376 & 0.400 & \subbst{0.172} & \subbst{0.267} & \bst{0.249} & 0.276  \\
    0.02 & 0.376 & 0.400 & 0.174 & 0.269 & \subbst{0.249} & 0.276  \\
    0.05 & \bst{0.375} & \subbst{0.399} & 0.174 & 0.268 & 0.252 & 0.278  \\
    0.1 & \subbst{0.375} & \bst{0.399} & 0.174 & 0.269 & 0.254 & 0.280  \\
    0.2 & 0.376 & 0.399 & 0.177 & 0.270 & 0.258 & 0.282  \\
    0.5 & 0.378 & 0.400 & 0.186 & 0.277 & 0.261 & 0.285  \\
    1 & 0.381 & 0.402 & 0.197 & 0.282 & 0.265 & 0.286  \\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \item  \tiny \textit{Note}: \bst{Bold} and \subbst{underlined} denote the best and second-best results.
    \end{tablenotes}
\end{threeparttable}
\end{minipage}
\hfill
\begin{minipage}[t]{0.495\textwidth}
\makeatletter\def\@captype{table}
% \vspace{2mm}
\renewcommand{\arraystretch}{1} \setlength{\tabcolsep}{4.7pt} \scriptsize
\centering
\renewcommand{\multirowsetup}{\centering}
\begin{threeparttable}
\caption{Varying $\gamma$ results of Fredformer.}\label{tab:sensi-gamma}
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{$\gamma$} & \multicolumn{2}{c}{ETTh2} & \multicolumn{2}{c}{ECL} & \multicolumn{2}{c}{Weather} \\
    \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
    & MSE & MAE & MSE & MAE & MSE & MAE \\
    \midrule
    0 & 0.377 & 0.402 & 0.191 & 0.284 & 0.261 & 0.282  \\
    0.001 & 0.371 & 0.397 & 0.182 & \subbst{0.275} & \subbst{0.257} & \subbst{0.279}  \\
    0.002 & 0.372 & 0.398 & \bst{0.181} & \bst{0.274} & 0.257 & 0.279  \\
    0.005 & 0.372 & 0.398 & 0.182 & 0.275 & 0.257 & 0.280  \\
    0.01 & \subbst{0.370} & 0.397 & 0.183 & 0.275 & \bst{0.257} & \bst{0.279}  \\
    0.02 & \bst{0.369} & \bst{0.395} & \subbst{0.182} & 0.275 & 0.258 & 0.280  \\
    0.05 & 0.370 & \subbst{0.396} & 0.187 & 0.279 & 0.259 & 0.281  \\
    0.1 & 0.371 & 0.397 & 0.196 & 0.287 & 0.261 & 0.283  \\
    0.2 & 0.372 & 0.398 & 0.209 & 0.298 & 0.263 & 0.285  \\
    0.5 & 0.376 & 0.399 & 0.230 & 0.317 & 0.266 & 0.287  \\
    1 & 0.386 & 0.406 & 0.239 & 0.326 & 0.268 & 0.290  \\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \item  \tiny \textit{Note}: \bst{Bold} and \subbst{underlined} denote the best and second-best results.
    \end{tablenotes}
\end{threeparttable}
\end{minipage}
% \vspace{-3mm}
\end{table}


